Video Storytelling: Textual Summaries for Events

Bridging vision and natural language is a longstanding goal in computer vision and multimedia research. While earlier works focus on generating a single-sentence description for visual content, recent works have studied paragraph generation. In this work, we introduce the problem of video storytelling, which aims at generating coherent and succinct stories for long videos. Video storytelling introduces new challenges, mainly due to the diversity of the story and the length and complexity of the video. We propose novel methods to address the challenges. First, we propose a context-aware framework for multimodal embedding learning, where we design a Residual Bidirectional Recurrent Neural Network to leverage contextual information from past and future. Second, we propose a Narrator model to discover the underlying storyline. The Narrator is formulated as a reinforcement learning agent which is trained by directly optimizing the textual metric of the generated story. We evaluate our method on the Video Story dataset, a new dataset that we have collected to enable the study. We compare our method with multiple state-of-the-art baselines, and show that our method achieves better performance, in terms of quantitative measures and user study.

==> table/fig_full_example_2.tex <==
\begin{figure*}[!t]
 \centering
%   \begin{minipage}[t]{1\textwidth}
% 	\centerline{\includegraphics[width=\linewidth]{frame_wedding}}
%   \end{minipage}
%   \begin{minipage}{1\textwidth}
%   	\centerline{\includegraphics[width=0.84\linewidth]{story_wedding}}
%   	\vspace{2em}
%   \end{minipage}  
%   \begin{minipage}{1\textwidth}
%   	\centerline{\includegraphics[width=\linewidth]{frame_christmas}}
%   \end{minipage}
%   \begin{minipage}{1\textwidth}
%   	\centerline{\includegraphics[width=0.84\linewidth]{story_christmas}}
%   \end{minipage}
  \begin{minipage}[t]{1\textwidth}
		\centerline{\includegraphics[width=\linewidth]{example_wedding}}
		\vspace{2ex}
		\centerline{\includegraphics[width=\linewidth]{example_christmas}}
  \end{minipage}   
  \caption
{
	\small
	Example stories generated by the proposed method (ResBRNN-kNN+Narrator), two baselines (H-RNN and EMD), and a ground truth.
	The frames are handpicked from the set of clips proposed by Narrator and the ground truth example.
	\textcolor{ForestGreen}{Green} boxes highlight the frames from GT,
	\textcolor{orange}{orange} boxes highlight the frames from Narrator proposals,
	while \textcolor{Red}{red} boxes highlight frames shared by both. 
}
  \label{fig:full_example2}
 \end{figure*}

==> table/tbl_language.tex <==
\begin{table*}[!t]
	\caption
		{
		\small	
			Evaluation of story generation on Video Story test set.
			Upper part evaluates different methods for clip to story retrieval, and lower part evaluates different methods for clip selection
		}
	\label{tbl:language}
	%\vspace{-2ex}
	\small
	\begin{center}
	\begin{tabular}{l l|c c c c c c c} 
		\toprule		
		Clip to Story & Clip Selection &CIDEr& METEOR&ROUGE-L&BLEU-1& BLEU-2&BLEU-3& BLEU-4\\
		\midrule
		Random& \multirow{8}{*}{Pseudo-GT} &30.2 &13.1&21.4&43.1&23.1 & 10.0& 4.8\\	
		S2VT~\cite{Venugopalan_ICCV_2015}& &64.0&14.3 &28.6&63.3 & 40.6&24.6&15.4 \\
		H-RNN~\cite{Yu_CVPR_2016} & &64.6&15.5 &28.8&61.6&41.4 &\bf{26.3} &\bf{16.1}  \\
		CCA & &71.8 &16.5 &26.7 & 60.1 & 34.7& 11.8&10.1 \\
		EMB & & 88.8 & 19.1 & 28.9& 64.5 & 39.3 & 22.7 & 13.4  \\
		BRNN & & 81.0 &18.1 &28.3&61.4 &36.6 &20.3 &11.3 \\
		ResBRNN& & 94.3 & 19.6 & 29.7&66.0& 41.7& 24.3&14.7\\ 
		ResBRNN-kNN& & \bf{103.6} &\bf{20.1} &\bf{29.9} &\bf{69.1} &\bf{43.5}&26.1 &15.6  \\ 
		\midrule
		\multirow{5}{*}{ResBRNN-kNN} &Uniform& 89.9 &18.3 &28.0&65.7 &40.6 &23.2 &13.2 \\
		& vsLSTM~\cite{Zhang_ECCV_2016}&92.4&18.2 &28.2 &66.6 &41.5 &24.1 &13.6  \\
		& Narrator w/o $\Vec{x}$&92.1 & 18.5 & 28.3 &67.3&41.6 &24.5 &14.2 \\
		& Narrator w/o $f_l$&94.9 & 18.8 & 29.1 &\bf{69.1}&42.9 &25.2 &14.5 \\
		& Narrator &\bf{97.6} & \bf{19.2} & \bf{29.3} &68.9&\bf{43.0} &\bf{25.2} &\bf{15.0} \\
		\bottomrule
	\end{tabular}
	\end{center}
\end{table*}	


